BERMo: What can BERT learn from ELMo?

We propose BERMo, an architectural modification to BERT, which makes predictions based on a hierarchy of surface, syntactic and semantic language features. We use linear combination scheme proposed in Embeddings from Language Models (ELMo) to combine the scaled internal representations from different network depths. Our approach has two-fold benefits: (1) improved gradient flow for the downstream task as every layer has a direct connection to the gradients of the loss function and (2) increased representative power as the model no longer needs to copy the features learned in the shallower layer which are necessary for the downstream task. Further, our model has a negligible parameter overhead as there is a single scalar parameter associated with each layer in the network. Experiments on the probing task from SentEval dataset show that our model performs up to $4.65\%$ better in accuracy than the baseline with an average improvement of $2.67\%$ on the semantic tasks. When subject to compression techniques, we find that our model enables stable pruning for compressing small datasets like SST-2, where the BERT model commonly diverges. We observe that our approach converges $1.67\times$ and $1.15\times$ faster than the baseline on MNLI and QQP tasks from GLUE dataset. Moreover, our results show that our approach can obtain better parameter efficiency for penalty based pruning approaches on QQP task.

==> Sections/experiment.tex <==

\section{Experimental Setup} \label{sec:experiment}
    In our experiments we consider BERT-based-uncased\footnote{\url{https://huggingface.co/bert-base-uncased}} as our baseline model which roughly contains 132M parameters. Our experiments are built on top of Movement Pruning Repository by huggingface (\cite{movement-pruning})\footnote{\url{https://github.com/huggingface/block_movement_pruning}}. Detailed list of hyperparameters for all the experiments can be found in Appendix \ref{apx:hyperparameters}. We found that higher learning rates for the skip connections improved the performance of the model and hence the learning rate for the skip connections was kept same as the masked learning rate ($10^{-2}$). 
    We run all our experiments with on RTX 2080 Ti having Intel Xeon Silver 4114 CPU (2.20 GHz). For all the task we use a single card, except for SQuAD simulations where we use of 2 cards to support higher sequence length.
    
    
\subsection{Datasets}
\par 
    As we combine the features from different depths to obtain a rich representation, we follow \cite{bert-language-structure} and evaluate our model on the probing tasks from the SentEval dataset (\cite{probing}). Tasks of this dataset are categorised into Surface (Sentence Length, Word content), Sytactic (Treedepth, Topconstant, and Bshift) and Semantic (Tense, subjnum, objnum, somo and coordinv) tasks helping us examine what linguistic tasks benefit from the BERMo architecture. Further, all the tasks of this dataset have 100k training, 10k validation and 10k testing samples with each class having identical number of samples. These properties of the dataset allow us to compare the raw accuracies of the model without worrying about the data imbalance issue.  
    
    In our experiments we observed that the baseline model commonly diverged for some of the probing tasks, when we subject the model to the compression.  
    Therefore, for the pruning task we evaluate our approach on MNLI and QQP tasks from the General Language Evaluation and Understanding (GLUE) dataset (\cite{glue}) and Stanford Question Answering (SQuAD) dataset (\cite{squad1.1}) to be comparable to (\cite{movement-pruning}). 
    Further, we test our model with SST-2 task from the GLUE dataset to verify our approach is also compatible with smaller datasets. 
    For comparing the model performance we use the F1 score for SQuAD, accuracy and F1 score for QQP, accuracy for MNLI and accuracy for SST-2.
    
\iffalse
\subsection{Simulations}


    
\subsection{Fine-Tuning}


\par
    For finetuning experiments on the probing task we train the model for 3 epochs with 5 randomly chosen seeds and report the mean and standard deviations. These experiments were run on a single card of Nvidia RTX 2080 Ti with a batch size of 32, sequence length of 128, 12000 warmup steps and a learning rate of $3\times10^{-5}$.
    
    %The models are trained 6 epochs with a batch size of 32 on a single NVIDIA GeForce \textcolor{red}{2080Ti}.
    
    We explore three training schemes in this work which we call hot, luke and cold. In the hot case all the weights including the pretrained weights of the BERT model are trainable.
    In the case of cold only the skip connections are trainable while luke allows the gradient flow and parameter updates for the pretrained BERT weights through the non skip paths.
    
    We use movementum-pruning with the hyperparameters in \cite{movement-pruning}. We purne the model for retaining $10\%$ of the initial weights.

\fi

